Fiduciary Responsibility: Facilitating Public Trust in Automated Decision Making

Automated decision-making systems are being increasingly deployed and affect the public in a multitude of positive and negative ways. Governmental and private institutions use these systems to process information according to certain human-devised rules in order to address social problems or organizational challenges. Both research and real-world experience indicate that the public lacks trust in automated decision-making systems and the institutions that deploy them. The recreancy theorem argues that the public is more likely to trust and support decisions made or influenced by automated decision-making systems if the institutions that administer them meet their fiduciary responsibility. However, often the public is never informed of how these systems operate and resultant institutional decisions are made. A ``black box'' effect of automated decision-making systems reduces the public's perceptions of integrity and trustworthiness. The result is that the public loses the capacity to identify, challenge, and rectify unfairness or the costs associated with the loss of public goods or benefits. The current position paper defines and explains the role of fiduciary responsibility within an automated decision-making system. We formulate an automated decision-making system as a data science lifecycle (DSL) and examine the implications of fiduciary responsibility within the context of the DSL. Fiduciary responsibility within DSLs provides a methodology for addressing the public's lack of trust in automated decision-making systems and the institutions that employ them to make decisions affecting the public. We posit that fiduciary responsibility manifests in several contexts of a DSL, each of which requires its own mitigation of sources of mistrust. To instantiate fiduciary responsibility, a Los Angeles Police Department (LAPD) predictive policing case study is examined.

==> extras.tex <==


Section 2:

competence and integrity, also known as fiduciary responsibility. The current paper examines the recreancy theorem in the context of automated decision-making systems’ DSLs. Investigations of recreancy explore public understandings of the integrity and trustworthiness of societal institutions’ behavior as they design, model, and implement automated decision-making systems in social landscapes (see \cite{sapp2021public}). The recreancy theorem is a useful framework for examining DSLs as methods of data collection, data modeling, and prediction output influence whether the public will perceive societal institutions and their use of AI innovations as trustworthy and honest. 


The degree to which the public trusts societal institutions in their administration of automated decision-making systems often affects whether they are permanently adopted or utilized long-term \cite{sapp2009consumer,sapp2021public}.




The public expects societal institutions to act with competency (i.e. skill, experience) and fiduciary responsibility  \cite{sapp2021public}. According to the recreancy theorem  \cite{sapp2009consumer}, public perceptions of public- and private-sector societal institutions’ fiduciary responsibility influence trust in and support for innovations (such as AI) administered by these organizations \cite{sapp2021public}. 



As described in \cite{sapp2021public}, the recreancy theorem postulates that societal institutions are more likely to be perceived as competent and reliable when the technological innovations they administer are perceived as effective, relevant, addressing self-interests, and minimizing negative effects on social justice for marginalized/vulnerable populations. 


, also known as fiduciary responsibility \cite{freudenburg1993risk}. That is, people's perceptions of institutional actors’ competence and fiduciary responsibility influence their ''trust in and support for [technological/AI] innovations administered by these institutions'' \cite[Pg. 2]{sapp2021public}. Research suggests that citizen trust in societal institutions depends on three central components: public perceptions of social institutions’ (1) competence, (2) integrity, and (3) benevolence (i.e. the extent to which the institution is concerned about citizens' welfare) \cite{cooper2008importance, kim2012participation, sapp2021public, schoorman2007integrative}. 


Trust in and support for public and private institutions' use of technological innovations requires institutional actors to behave in a manner that gives citizens reason to believe in their performance, and is established through a perceived bond between the public and the institutions that serve them \cite{freudenburg1993risk,sapp2021public}. 





We will consider a case study in Section \ref{sec:case} of predictive policing technology deployed by the Los Angeles Police Department (LAPD).  Our analysis will show that the LAPD failed to meet their fiduciary responsibility, in part, by not adequately communicating with the public the stages of the data science lifecycle.  Thus, the recreancy theorem, particularly in the context of data science lifecycles, provides a framework for combatting the phenomenon that is sometimes referred to as the ``black box'' effect \cite{european2020white,wachter2017counterfactual}.







==> responsibility.tex <==
% Section on Fiduciary Responsibility and Trust

%ERIC - RECOMMEND CUTTING THESE TWO PARAGRAPHS AND CHANGING SECTION HEADING TO "CONCEPTUAL FRAMEWORK"

Multiple scholars argue that when societal institutions with varying roles and responsibilities fail to build trust among the populations they serve (i.e. reflect recreancy), society’s ability to function is detrimentally affected  \cite{roth1978economy,freudenburg1993risk,alario2003paradoxes,sapp2021public}. Some have argued that trustworthiness, not trust, denotes public judgments of societal institutions’ behaviors \cite{colquitt2007trust,ball2019institutional,sapp2021public}. Sapp et al. \cite{sapp2021public} (see also \cite{freudenburg1993risk}) defines trustworthiness as behaviors by societal institutions that give citizens reason to place faith in their performance. 

When the public perceives a societal institution as meeting their expectations of competent and trustworthy performance, interpersonal trust between the two is established  \cite{deutsch1958trust,barber1983logic,sapp2021public}. This form of trust is initiated through the perceived competence, benevolence, and ethics of institutional behavior  \cite{barber1983logic,hardin2001conceptions,blomqvist2005playing,sapp2021public}, and past research affirms this contention  \cite{kim2012participation,ball2019institutional,sapp2021public}. Public perceptions of competence and integrity effectively explain the trust in and support for societal institutions  \cite{sapp2009consumer,sapp-dm2009consumer,sapp2021public}. Indeed, previous research shows that public opinions of these institutions can alter trust in and support for technological innovations that they administer in public spaces  \cite{earle1995social,siegrist2000perception,sapp2021public}, such as automated decision-making systems. 

\subsection{The Recreancy Theorem} \label{ssec:recreancy}

As conceptualized by Sapp et al. \cite{sapp2009consumer}, the recreancy theorem argues that the public’s trust in public and private societal institutions is explained by their assessments of institutional actors' competence (i.e. skill, ability, experience), and their confidence that these actors will behave with integrity (i.e. honesty, ethical standards), also known as fiduciary responsibility \cite{freudenburg1993risk}. Benevolence is a third central component of public trust, which involves the perceived extent to which the institution is concerned about citizens' welfare). 

Sapp et al. \cite{sapp2021public} (see also \cite{freudenburg1993risk}) define trustworthiness as institutional behaviors that give citizens reason to have confidence in their performance. Interpersonal trust is embedded in the recreancy theorem wherein there is a perceived connection between a societal institution and individuals in the population they serve \cite{sapp2021public}. When the public perceives an institution as meeting their expectations of competent, honorable, and benevolent performance, interpersonal trust between the two is established \cite{barber1983logic,blomqvist2005trust,deutsch1958trust,sapp2021public}, and past research affirms this contention  \cite{ball2019institutional,kim2012participation,sapp2021public}. Such assessments influence whether the public trusts and supports technological innovations, such as algorithm-driven automated decision-making systems DSLs, proposed or administered by these institutions \cite{barber1983logic,blomqvist2005trust,hardin2001conceptions}). Additionally, recent research reveals that the public is more likely to trust social institutions when their newly administered AI does not negatively affect social justice--i.e. protects the interests of vulnerable/marginalized populations \cite{cooper2008importance,kim2012participation,sapp2021public,schoorman2007integrative}. The degree to which the public trusts institutions in their administration of DSLs often affects whether those systems are discarded or used long-term \cite{sapp2009consumer,sapp2021public}.

In the current paper, we specifically focus on fiduciary responsibility in societal institutions’ development and administration of DSLs, as methods of data collection, data modeling, and prediction output influence whether the public will perceive those establishments as having integrity. Multiple scholars have argued that when societal institutions (with a wide spectrum of roles and responsibilities) fail to build trust among the populations they serve (i.e. reflect recreancy), society’s ability to function is detrimentally effected \cite{alario2003paradoxes, freudenburg1993risk,roth1978economy,sapp2021public}. Public perceptions of institutions’ fiduciary responsibility influence trust in and support for DSLs administered by these organizations \cite{sapp2021public}.

\subsection{Fiduciary Responsibility}

Fiduciary responsibility \cite{sapp2021public} is an integral tenet of the recreancy theorem and refers to public perceptions of the integrity demonstrated by societal institutions, which affects individuals’ trust in and support for automated decision-making systems administered by those institutions. Data scientists (internal or external to public and private institutions) are often those who develop (i.e. perform data collection and data modeling) the algorithms driving these systems in collaboration with the societal institutions that eventually administer them in the public sphere. This process can be conceptualized as the DSL. We endeavor to show that the DSL typically operates within a “black box” where data scientists and institutional staff make system development and administration decisions “in the dark” absent public technological knowledge, understanding, and scrutiny, which hinders the perceived fairness of those technologies once they are administered. 

Scholarship suggests that institutional administration of AI raises multiple concerns specific to integrity, including invasion of privacy, loss of personal health data, and unfair monitoring or targeting of particular individuals or groups, which may sometimes involve racial bias \cite{anderson2018artificial,hitlin2019facebook,olmstead2017americans,rainie2017code, rainie2017internet,sapp2021public}. Perceptions of institutional integrity thus depends on whether the public believes automated decision-making systems are ethically administered – e.g. protect individuals from disadvantage and unjust treatment in society \cite{ball2019institutional,kim2012participation,sapp2021public} across the DSL. Societal institutions that administer algorithm-driven automated decision-making systems with honor – e.g. concern for and attention toward minimizing biased/racist impacts and privacy infringement – are more likely to be trusted by the public \cite{sapp2021public}.

\subsection{The Recreancy Theorem and Public Trust in Technical Innovations} \label{ssec:innovations}

The recreancy theorem, as applied specifically to technical innovations, delineates three dimensions of public acceptance of technical innovations.  As stated in \cite{sapp2021public}, the recreancy theorem
\begin{quote}
complements technology adoption models in that it focuses upon public assessments of innovations as they are managed by societal institutions, thereby providing conceptual congruity between technology adoption and public assessments of institutional competency and integrity. 
\end{quote}

To that end, \cite{sapp2009consumer,sapp2013science} argues that the public is more likely to trust and accept the implementation and use of technologies that pose a risk to their welfare or interests provided they meet the following requirements.  First, they (the technologies and/or institutions deploying those technologies) must possess \textbf{technical competency}, meaning that they must have the capability to perform the analysis and/or actions required for the intended purpose of the technologies. Second, they must have a \textbf{public benefit}, meaning that these technologies should improve upon a specific problem of public concern upon deployment. And third, they must meet \textbf{fiduciary responsibility}, meaning that the algorithms are designed and employed with integrity, and are in fact performing in the way that they are intended, without disparate impacts or misuse by agents.  

Each of these dimensions warrants investigation with respect to the public's trust in AI deployment, in particular.  We describe in Subsection \ref{ssec:related} prior works that have related themes, especially methods for formalizing, analyzing, and quantifying technical competency. As such, we will not address that dimension here, nor will we consider the public benefit aspect of the recreancy theorem.  We will focus on fiduciary responsibility, building upon recent research findings that fiduciary responsibility is of particular importance among the public, especially for the protection of vulnerable populations.

The application of AI innovations addresses public self-interests when it protects individuals from detrimental outcomes such as privacy infringement, loan or credit denial, identity theft, etc. \cite{sapp2021public}. Scholarship suggests that institutional administration of technological innovations raises multiple concerns specific to integrity, including invasion of privacy, loss of personal health data, and unfair monitoring or targeting of particular individuals or groups, which may sometimes involve racial bias \cite{anderson2018artificial, hitlin2019facebook, olmstead2017americans, rainie2017code, rainie2017internet, sapp2021public}. Perceptions of institutional integrity thus depends on whether the public believes AI innovations are ethically administered--i.e. protect individuals from disadvantage and unjust identity-based treatment in society \cite{ball2019institutional, kim2012participation}.

Further, \cite{sapp2021public} discusses a conceptual understanding of public opinions of network surveillance and empirically documents public demand for network surveillance that fosters goals of social justice more so than goals of self-interest.  The findings are based on a nationwide survey of adults concerning governments' use of network surveillance.  Additionally, the utilization of a technological innovation is often perceived as socially just when it protects the rights of marginalized/vulnerable populations such as people of color, women, and LGBTQ+ individuals \cite{sapp2021public}.

%Because of this recent work, the focus of the present paper is the fiduciary responsibility of deployment of data science lifecycles.

The recreancy theorem asserts that the public's acceptance of technical innovations depends on the public's perception that fiduciary responsibility is being met by institutions deploying those technologies.  Therefore, it is incumbent upon institutions to ensure that the public is confident that fiduciary responsibility is met by the technologies in use.  By utilizing the formalism of a data science lifecycle, we argue that this can best be done through transparency at multiple stages of the lifecycle, especially those stages occurring in the third layer (see Figures 1 and 2) that we identify as interpretation and communication.

%We use ``public'' in a manner similar to that in \cite{knowles2021sanction}: average, relatively non-technical citizens who have a stake in, or are subject to, automated decision making systems.

%We use ``trust'' in a colloquial manner, rather than a technical manner.  Discuss various ways to describe trust in technical innovations.

\subsection{Related Work} \label{ssec:related}

Public trust in automated decision making systems or artificial intelligence is, \emph{prima facie}, both important to establish and difficult to formalize.  For example, \cite{lewis1985trust,hofstede2006intrinsic,WHKA14} formalize trust, either interpersonal or institutional.  Several high profile institutions, \cite{ibm2020trusting,european2020white} just to name a few, acknowledge the importance of establishing trust in AI while using the term in a colloquial sense.  Early efforts to formalize trust in various forms of digital interactions appear in \cite{YH08,harper2014trust}.

Recent work has endeavored to describe trust in AI in several different ways on a technical basis.  Several authors have posited a formal definition of trust in AI by drawing on prior work in formalizing interpersonal and institutional trust.  Other authors have proposed methods for quantifying, or establishing, trust through established legal or public policy structures.  Still others have distinguished between trust in AI versus trustworthy AI.  There are multiple ways in which our use of the recreancy theorem in general, and fiduciary responsibility in particular, in the context of public trust in AI are related to these other works.  We describe those relations here.

It is well understood that public trust in AI has multiple dimensions. The three facets of the recreancy theorem--competency, benefit, and fiduciary responsibility--are reflected in others' investigations into the question of how AI can be trustworthy.  Indeed, \cite{jobin2019global} finds similar dimensions as the recreancy theorem:
\begin{quote}
To investigate whether a global agreement on these questions is emerging, we mapped and analyzed the current corpus of principles and guidelines on ethical AI. Our results reveal a global convergence emerging around five ethical principles (transparency, justice and fairness, non-maleficence, responsibility and privacy), with substantive divergence in relation to how these principles are interpreted.
\end{quote}
Toreini et al. \cite{toreini2020relationship} describe trust in AI as distinct from trustworthy ML by utilizing the ABI framework--Ability, Benevolence, and Integrity--posited by \cite{mayer1995integrative} to model organizational trust.  We note that Mayer's ABI framework and the recreancy theorem run parallel to each other in their dimensions, while the notion of trustworthy as a part of trust as formulated by Toreini et al. reflect the technical competency of the recreancy theorem.  This is borne out by several related notions such as trustworthy AI and human-AI trust.

In general, \emph{trustworthy AI} refers to the competence of the AI algorithm, with competence defined in terms of a contract.  This is precisely how Jacovi et. al. \cite{jacovi2021formalizing} define the notion: ``an AI model is trustworthy to some contract if it is capable of maintaining this contract.''  Similarly, \cite{hawley2014trust} describes trust facilitated through a  commitment (i.e. a contract); this commitment also involves expectations by the trustor about the competence and willingness of the trustee.  Knowles et. al. \cite{knowles2021sanction} develop a foundation for trust in AI through a transparent and understandable regulatory system.  
%They argue that 
%\begin{quote}
%    a lack of public trust in AI has little to do with people's inability to understand how AIs work; rather it is a response to an awareness of a lack of structural assurances of the trustworthiness of the AIs pervading society.
%\end{quote}
They argue that a regulatory system can potentially bridge the gap between trustworthy and trust.  Such a regulatory system can be a mechanism for extending the public's trust from its acceptance that a particular AI meets the required technical competence to meeting the required fiduciary responsibility as well.


Jacovi et. al. \cite{jacovi2021formalizing} further propose a formal definition of \emph{human-AI} trust via adapting the sociological definition of interpersonal trust.  The definition has several dimensions, including trustworthiness of the algorithm and warranted trust possessed by the human who is at risk of the AI's actions.  They posit that an algorithm is trustworthy if it can uphold a contract, and a human possesses warranted trust of AI if the human has reason to accurately anticipate the impact of the AI's decisions.  The notion of trustworthy put forth in \cite{jacovi2021formalizing} need not require an individual to understand the inner-workings of the algorithm.

Others have argued for facilitating public trust in AI through an understanding of the workings of the algorithms, whether by individuals that are subject to AI or by experts who can vouch for the competency of the algorithms.  A large body of literature discusses Explainable AI (XAI) as one method for ensuring trust between users and AI \cite{ribeiro2016should,mittelstadt2019explaining}.  Documentation, such as AI factsheets \cite{arnold2019factsheets,richards2020methodology} (for example the European requirements for factsheets \cite{european2020white}) or declarations of conformity \cite{hind2018increasing}, is a potential way to build public trust by facilitating auditing of AI.  Both of these mechanisms are designed to establish the perception of the technical competency of the algorithms among the public.












%IDEA: contract or commitment, i.e. competency  CONNECTION BETWEEN FIDUCIARY RESPONSIBILITY AND CONTRACT.


%\cite{richards2020methodology} AI Factsheets
%
%IDEA: understandable and/or trustworthy algorithms; Competency
%
%again, factsheets.


%MOVE SOME OF THESE TO FIRST PARAGRAPH.  OLDER PAPERS, FOUNDATIONAL RESULTS, HISTORICAL RECORD, IMPORTANT PROBLEM.

%\cite{kroeger2017facework} creating trust in systems


%\cite{hoffman2017taxonomy} a view of human trust in machines that regards trusting as a process, that emphasizes dynamics over states, and that distinguishes a considerable variety of trusting relationships











%DONE:
%
%
%\cite{hofstede2006intrinsic} intrinsic or enforceable trust
%\cite{lewis1985trust} formalizes interpersonal trust and extension to communities
%\cite{WHKA14} trust-based decision making
%
%\cite{YH08} model of trust for digital systems
%
%\cite{harper2014trust} trust in a technical sense -- multiple discussions to formalize trust in computing technology


